SkillWrapper: Generative Predicate Invention for Task-level Robot Planning

Generalizing from individual skill executions to long-horizon tasks is a core challenge in building autonomous robots. A promising direction is learning high-level, symbolic representations of low-level robot skills, enabling abstract reasoning independent of the low-level state space. Recent advances in foundation models have made it possible to generate symbolic predicates that operate on raw sensory inputs-a process we call generative predicate invention-to facilitate downstream representation learning. However, prior work learns these abstractions using heuristic or ad-hoc procedures, leaving unclear which formal properties they ought to satisfy, and how these properties can guide representation learning. We address these questions by characterizing conditions under which learned representations support sound and complete task-level planning, and using them to guide the design of SkillWrapper, a system that autonomously learns symbolic representations of black-box skills without predefined tasks, predicates, or operators. Our approach leverages foundation models to actively collect robot data and learn human-interpretable, plannable representations directly from RGB observations. Our extensive empirical evaluation in simulation and on real robots shows that SkillWrapper learns abstract representations that enable robots to compose black-box skills to solve unseen, long-horizon tasks in the real world.

==> sections/formal_framework.tex <==
We consider a problem setting in which a robot is equipped with an inventory of predefined, ``black-box'' skills.
%
The robot can evaluate whether a given skill is executable in the current state, but does not have a transition model of the effects of executing the skill.


%
The agent can evaluate whether a skill is executable in the current state, but it does not have a \textcolor{red}{complete} transition model of the skills a priori,
%
and therefore cannot compose its skills to solve long-horizon problems without considering low-level details.
%
However, if the agent were to learn symbolic models of its skills, it could use classical planning to efficiently compose them to solve new tasks.
%
%This        We - Kept for comment
%
In this section, we formalize this setting as the problem of \emph{Skill Model Learning}.
%, and define the concepts required to understand our method.
% learning \emph{Skill Abstraction}s.
%
% We then define formal properties that any method for active skill abstraction might aim to achieve.

\subsubsection{Preliminaries}

\paragraph{Environment Model.}{
    % As the agent learns to compose its skills across a range of settings, the agent itself and its skills remain the same.
    % %
    % Consequently, our model differentiates between aspects of the problem that remain the same---the \emph{environment}---and those that vary between different \emph{settings}.
    % %
    %Formally, 
    We define an \emph{environment} as a tuple $\DefDomain$, where the \emph{state space} $\States$ is assumed to be high-dimensional, continuous, and fully observable; %(i.e., each state $s \in \mathbb{R}^n$).
    %
    the \emph{type set} $\Types$ enumerates the possible object types;
    %
    and the \emph{skills} $\Skills$ are object-centric, such that each $\skill \in \Skills$ is parameterized by object types drawn from the \emph{type set} $\Types$.
    %
    The \emph{transition function} $\DefTransitionFunction$ characterizes the environment dynamics but is unknown to the agent.
% The agent is equipped with \emph{object-centric skills} $\skill \in \Skills$ parameterized by object types drawn from the \emph{type set} $\Types$.
    % %
    % The agent is equipped with \emph{object-centric skills} $\skill \in \Skills$ parameterized by object types drawn from the \emph{type set} $\Types$.
    %
    For example, \texttt{Pour(?teapot,}~\texttt{?mug)} may be used to pour tea from a teapot into a mug.
    %
    However, certain environmental aspects (e.g., which mugs are available to pour into) may differ between settings during learning.
    %
    We therefore define a specific \emph{setting} by the tuple $\DefSetting$, specifying an initial state $\initialState \in \States$ and a set of typed objects $\Objects$, where the type(s) of object $\object \in \Objects$ are denoted by $\typeOf{\object} \subseteq \Types$.
    %
    % shared across all environments... (on the set of skills)
}\label{sec:environment-model}

\paragraph{Black-box Skills.}{
    We model skills as object-centric options~\citep{sutton1999options} with discrete, object-typed parameters.
    %
    Formally, a \emph{skill} $\skill \in \Skills$ is defined by a tuple $\DefSkill$,
    %
    where the \emph{initiation set} $\InitiationSetOf{\skill} \subseteq \States$ contains states from which the skill may be executed;
    %
    the \emph{policy}~$\OptionPolicy$ controls the agent during the skill;
    %
    the \emph{termination set} $\TerminationSet \subseteq \States$ is the set of states at which the skill immediately terminates;
    %
    and the \emph{skill parameters} $\DefParametersOf{\skill}{k}$ specify type constraints $\typeOf{\parameterOf{\skill}^i} \subseteq \Types$ for valid skill arguments.
    %
    Specifically, a skill $\skill \in \Skills$ may be instantiated to create a \emph{skill instance} $\skillInstance$ using objects $\NTupleOf{k}{\object} \in \Objects^k$ if and only if for $1 \leq i \leq k$, $\typeOf{\parameterOf{\skill}^i} \subseteq \typeOf{\object_i}$.
    %
    We assume that executing a skill only affects the state of objects passed as arguments.\footnote{We do not, however, assume that a skill necessarily affects the state of \emph{all} objects passed in as arguments.}
}

\paragraph{Symbolic Abstractions.}
% \textcolor{red}{did we say we only consider less than 2-arity predicates?}
%
Because the agent must evaluate $\InitiationSetOf{\skill}$ on individual states, it cannot distinguish essential skill information from irrelevant details, making long-horizon planning combinatorially difficult.
%
%, as each state is treated as a separate atomic entity.
%
However, each skill affects only a few objects at once, leaving the rest of the world unchanged.
%
The agent can exploit this property by instead learning a factored state representation---formalized here as first-order logic models in PDDL~\citep{mcdermott1998pddl}---providing an abstract transition model of its skills.
%
Such abstractions enable the agent to use classical planning to compose its skills and accomplish unseen, long-horizon goals.


We use symbolic \emph{predicates} $\Predicates$ to express abstract relations between objects.
%
Each predicate $\predicate \in \Predicates$ is a tuple $\DefPredicate$, where the \emph{predicate classifier} $\PredicateClassifier$ tests whether the predicate holds in a state, given a binding of objects to the \emph{predicate parameters} $\DefParametersOf{\predicate}{n}$.
%
Each parameter $\parameterOf{\predicate}^i$ specifies a type constraint $\typeOf{\parameterOf{\predicate}^i} \subseteq \Types$ on corresponding object arguments.
%
Formally, the partial function\footnote{We denote a partial function using $f:\mathcal{X} \rightharpoonup \mathcal{Y}$.}
%
\mbox{$\DefPredicateClassifier$} is defined on objects $\NTupleOf{n}{\object} \in \Objects^n$ if and only if $\typeOf{\parameterOf{\predicate}^i} \subseteq \typeOf{\object_i}$ for $1 \leq i \leq n$.
%
In such cases, we say that the objects $\NTupleOf{n}{\object}$ are \emph{valid arguments} for $\predicate$.

%
% Comment
%

% Using the invented predicates $\Predicates$, the learning method must construct a set of \textit{operators} (i.e., relational abstract actions) defining abstract transition models for the agent's skills. 
By observing different effects, the agent must construct a set of \textit{operators} $\Operators$ that define abstract transition models for the agent's skills.
%
% These transition models are represented using the set of predicates $\Predicates$.
%
We define each operator $\operator \in \Operators$ by $\DefOperator$, 
%
where $\operatorSkill \in \Skills$ is the corresponding skill;
%
the \emph{operator parameters} $\DefParametersOf{\operator}{m}$ impose type constraints $\typeOf{\parameterOf{\operator}^i} \subseteq \Types$ on operator arguments;
%
the \emph{preconditions} $\PRE$ are a conjunction of literals over $\Predicates$ defining the conditions necessary to apply the operator;
%
and the \emph{add} and \emph{delete effects}, $\AddEFF$ and $\DeleteEFF$, are the subsets of $\Predicates$ that become true and false, respectively, after the operator is applied.

\paragraph{Grounded Abstractions.} To apply an abstract transition model to a real-world setting, the agent must map the low-level state to an abstract state, which requires \emph{grounding} the known predicates using concrete objects so that their truth value may be determined.
%
% To apply the abstract transition model to a real-world setting, an agent needs to appropriately map the state of the real world to an abstract state, which requires determining the truth value of known predicates.
%
A predicate $\predicate \in \Predicates$ may only be grounded using valid arguments, inducing a \emph{grounded predicate} $\DefGroundedPredicate$.
%
Given a low-level state, the classifier \mbox{$\DefGroundedPredicateClassifier$} tests whether the predicate holds for the object arguments.
%
% We can evaluate whether a predicate $\predicate \in \Predicates$ holds for specific objects $\object_{1:n} \in \Objects$ in a state $\state \in \States$ by first \emph{grounding} the predicate by binding the objects comprising that state to the predicate parameters $\ParametersOf{\predicate}$.
%
We define the set of \emph{grounded predicates} for a setting $\DefSetting$ under predicates $\Predicates$ as \mbox{$\DefGroundedPredicates$}, inducing an \emph{abstract state space} $\DefAbstractStates$ where each abstract state corresponds to a specific combination of grounded relations.

% The \emph{abstraction function} $\DefAbstractionFunction$ formalizes this relationship by mapping each low-level state $\state \in \States$ to an abstract state $\abstractState \in \AbstractStates$ corresponding to the subset of grounded predicates true in the state.

% \begin{equation}
%     \abstractState = \AbstractionFunction(\state) \triangleq \{ \groundedPredicate \; | \; \groundedPredicate \in \GroundedPredicates \land \GroundedPredicateClassifier(\state) = 1 \}.
% \end{equation}

% David had suggested adding:  where each abstract action corresponds to a black-box skill,

Given a set of operators $\Operators$ in a setting $\DefSetting$, the \emph{abstract action space} $\AbstractActions$ is the set of all valid groundings of the operators using objects from $\Objects$.
%
% The \emph{abstract action space} $\AbstractActions$ is similarly defined by grounding each operator $\operator \in \Operators$ using all valid combinations of objects in the environment.
%
Each \emph{abstract action} (i.e., grounded operator) is defined as $\DefAbstractAction$, where $\operator \in \Operators$, $\NTupleOf{m}{\object} \in \Objects^m$, and for $1 \leq i \leq m$, $\typeOf{\parameterOf{\operator}^i} \subseteq \typeOf{\object_i}$.
%
Grounding an operator induces \emph{ground preconditions} $\GroundPRE$, which are a conjunction of ground literals over $\GroundedPredicates$;
\emph{ground add effects} $\GroundAddEFF \subseteq \GroundedPredicates$;
and \emph{ground delete effects} $\GroundDeleteEFF \subseteq \GroundedPredicates$.

%To express relationships between symbolic abstractions and low-level states
The \emph{grounding function} $\Grounding: \GroundedPredicates \to 2^\States$ maps each grounded predicate to its \emph{grounding set} $\GroundingSetOf{\groundedPredicate} \subseteq \States$, defined as \mbox{$\DefGroundingSet$}.
%
% the set of states in which the grounded predicate is true.
%
We overload this notation for abstract states $\abstractState \in \AbstractStates$ so that \mbox{$\GroundingSetOf{\abstractState} \Def \bigcap_{\groundedPredicate_i \in \abstractState} \GroundingSetOf{\groundedPredicate_i}$}.
%
Conversely, the \emph{abstraction function} $\DefAbstractionFunction$ maps each low-level state $\state \in \States$ to the abstract state $\abstractState \in \AbstractStates$ defined by \mbox{$\AbstractionFunction(\state) \Def \Set{\groundedPredicate \in \GroundedPredicates \SetSuchThat \GroundedPredicateClassifier(\state) = 1}$}.

% An \emph{abstraction function} $\DefAbstractionFunction$ maps each low-level state $\state \in \States$ to an abstract state $\abstractState \in \AbstractStates$ corresponding to the subset of grounded predicates true in the state:

% \begin{equation}
%     \abstractState = \AbstractionFunction(\state) \triangleq \{ \groundedPredicate \; | \; \groundedPredicate \in \GroundedPredicates \land \GroundedPredicateClassifier(\state) = 1 \}.
% \end{equation}

% the \emph{grounding} of an abstract state is the set of low-level states in which all grounded predicates in the abstract state hold.
%
%Finally, the grounding of a set of grounded predicates is the set of low-level states in which all grounded predicates in the set are true.

% $\GroundingSet{\abstractState} = \{ s \in \States \,:\, \forall \groundedPredicate \in \abstractState, \groundedPredicate(s) = 1 \}$

% \textcolor{red}{(Might not be useful anymore since we don't talk about disjunctiveness)In our setting, we assume to have access to a predicate generator $\mathbf{G}$ that proposes predicates $\mathcal{P}$ conditioned on $X \in \mathcal{S}$, such that $\mathcal{G}(\hat{P}) = X$.}

% \subsection{Active Skill Abstraction}
% One aspect that distinguishes our method from Nishanth's papers is the active learning paradigm...

\subsubsection{Problem Definition}
\begin{definition}
Given an environment $\DefDomain$ containing settings $\{ \DefSetting \}_{i=1}^N$, we define a \emph{Skill Model Learning} problem as learning an \emph{abstract transition model} $\DefModel$ for the skills $\Skills$.
\end{definition}

After a period of continual learning in one or more settings, an agent may be evaluated on an \emph{skill planning problem} $\DefPlanningProblem$, where $\DefGoalStates$ is the set of \emph{goal states} to be reached. 
%
Given a model $\DefModel$, a classical planner can be used to search for an \emph{abstract plan} $\DefAbstractPlan$ that solves the \emph{abstract planning problem} $\DefAbstractPlanningProblem$.
%
\begin{definition}
    An abstract plan $\DefAbstractPlan$ is called a \emph{solution} for skill planning problem \mbox{$\DefPlanningProblem$} iff %, letting $\skillInstance_i$ denote $\skillInstance_{\abstractAction_i}$,
    %
    for $1 \leq i \leq n,\, \state_{i} = \TransitionFunction(\state_{i-1}, \skillInstance_i),
    \state_{i-1} \in \InitiationSetOf{\skillInstance_i},
    \text{ and } \state_n \in \GoalStates,$
    where $\skillInstance_i = \skillInstance_{\abstractAction_i}$.
\end{definition}

% A \emph{solution} to the problem takes the form of a sequence of grounded operators that can map to a \emph{skill plan} (i.e., sequence of skill instances) $\DefPlan$ that reaches a goal state $s_n \in \GoalStates$ from the environment's initial state $\initialState \in \States$.

% \begin{definition}
%     Given an abstract transition model $\mathcal{M}=(\mathcal{P}, \mathcal{A})$ and a skill planning problem $\mathbf{p}$, an \emph{abstract planning problem} requires identifying an abstract plan $[\underline{a}_0, \dots, \underline{a}_{n-1}]$, where $a_i \in \mathcal{A}$, such that the corresponding skill plan $[\skillInstance_0, \dots, \skillInstance_{n-1}]$ is a solution to $\mathbf{p}$.
% \end{definition}

In Sec.~\ref{sec:skillwrapper}, we describe how {\sys} constructs $\gM$ from raw skill executions.


==> sections/full_formal_framework.tex <==
% In this section, we define our problem setting and the concepts required to understand our method.
%
We consider a problem setting in which a robot is equipped with a set of pre-existing, ``black-box'' skills.
%
The robot can evaluate whether a skill is executable in the current state, but it does not have a \textcolor{red}{complete transition model} of the skills a priori,
%
and therefore cannot compose its skills to solve long-horizon problems without considering low-level details.
%
However, if the robot were to learn a symbolic model of its skills, it could use classical planning approaches to efficiently compose its skills and enable the robot to solve novel tasks.
%
We formalize this setting as the problem of \emph{Task-Level Model Learning}.

\subsection{Preliminaries}

\paragraph{Environment model}{
    % As the robot learns to compose its skills across a range of settings, the robot itself and its skills remain the same.
    % %
    % Consequently, our model differentiates between aspects of the problem that remain the same---the \emph{environment}---and those that vary between different \emph{settings}.
    % %
    %Formally, 
    We define an \emph{environment} as a tuple $\DefDomain$, where the \emph{state space} $\States$ is assumed to be high-dimensional, continuous, and fully observable; %(i.e., each state $s \in \mathbb{R}^n$).
    %
    the \emph{type set} $\Types$ enumerates the possible object types;
    %
    and the \emph{skills} $\Skills$ are object-centric, such that each $\skill \in \Skills$ is parameterized by object types drawn from the \emph{type set} $\Types$.
    %
    The \emph{transition function} $\DefTransitionFunction$ characterizes the environment dynamics but is unknown to the robot.
% The robot is equipped with \emph{object-centric skills} $\skill \in \Skills$ parameterized by object types drawn from the \emph{type set} $\Types$.
    % %
    % The robot is equipped with \emph{object-centric skills} $\skill \in \Skills$ parameterized by object types drawn from the \emph{type set} $\Types$.
    %
    For example, \texttt{Pour(?teapot,}~\texttt{?mug)} may be used to pour tea from a teapot into a mug.
    %
    However, certain environmental aspects (e.g., which mugs are available to pour into) may differ between settings during learning.
    %
    We therefore define a specific \emph{setting} by the tuple $\DefSetting$, specifying an initial state $\initialState \in \States$ and a set of typed objects $\Objects$, where the type(s) of object $\object \in \Objects$ are denoted by $\typeOf{\object} \subseteq \Types$.
    %
    % shared across all environments... (on the set of skills)
}\label{sec:environment-model}

\paragraph{Black-box skills}{
    We model skills as object-centric options~\citep{sutton1999options} with discrete, object-typed parameters.
    %
    Formally, a \emph{skill} $\skill \in \Skills$ is defined by a tuple $\DefSkill$,
    %
    where the \emph{initiation set} $\InitiationSetOf{\skill} \subseteq \States$ contains states from which the skill may be executed;
    %
    the \emph{policy}~$\OptionPolicy$ controls the robot during the skill;
    %
    the \emph{termination set} $\TerminationSet \subseteq \States$ is the set of states at which the skill immediately terminates;
    %
    and the \emph{skill parameters} $\DefParametersOf{\skill}{k}$ specify type constraints $\typeOf{\parameterOf{\skill}^i} \subseteq \Types$ for valid skill arguments.
    %
    Specifically, a skill $\skill \in \Skills$ may be instantiated to create a \emph{skill instance} $\skillInstance$ using objects $\NTupleOf{k}{\object} \in \Objects^k$ if and only if for $1 \leq i \leq k$, $\typeOf{\parameterOf{\skill}^i} \subseteq \typeOf{\object_i}$.
    %
    We assume that executing a skill only affects the state of objects passed as arguments.\footnote{We do not, however, assume that a skill necessarily affects the state of \emph{all} objects passed in as arguments.}
}

\paragraph{Symbolic abstractions}
% \textcolor{red}{did we say we only consider less than 2-arity predicates?}
%
Because the robot must evaluate $\InitiationSetOf{\skill}$ on individual states, it cannot distinguish essential skill information from irrelevant details, making long-horizon planning combinatorially difficult.
%
%, as each state is treated as a separate atomic entity.
%
However, each skill affects only a few objects at once, leaving the rest of the world unchanged.
%
The robot can exploit this property by instead learning a factored state representation---formalized here as first-order logic models in PDDL~\citep{mcdermott1998pddl}---providing an abstract transition model of its skills.
%
Such abstractions enable the robot to use classical task planning to compose its skills and accomplish unseen, long-horizon goals.


We use symbolic \emph{predicates} $\Predicates$ to express abstract relations between objects.
%
Each predicate $\predicate \in \Predicates$ is a tuple $\DefPredicate$, where the \emph{predicate classifier} $\PredicateClassifier$ tests whether the predicate holds in a state, given a binding of objects to the \emph{predicate parameters} $\DefParametersOf{\predicate}{n}$.
%
Each parameter $\parameterOf{\predicate}^i$ specifies a type constraint $\typeOf{\parameterOf{\predicate}^i} \subseteq \Types$ on corresponding object arguments.
%
Formally, the partial function
% \footnote{We denote a partial function using $f:\mathcal{X} \rightharpoonup \mathcal{Y}$.}
%
\mbox{$\DefPredicateClassifier$} is defined on objects $\NTupleOf{n}{\object} \in \Objects^n$ if and only if $\typeOf{\parameterOf{\predicate}^i} \subseteq \typeOf{\object_i}$ for $1 \leq i \leq n$.
%
In such cases, we say that the objects $\NTupleOf{n}{\object}$ are \emph{valid arguments} for $\predicate$.

%
% Comment
%

% Using the invented predicates $\Predicates$, the learning method must construct a set of \textit{operators} (i.e., relational abstract actions) defining abstract transition models for the robot's skills. 
By observing different effects, the robot must construct a set of \textit{operators} $\Operators$ that define an abstract transition model for the robot's skills.
%
% These transition models are represented using the set of predicates $\Predicates$.
%
We define each operator $\operator \in \Operators$ by $\DefOperator$, 
%
where $\operatorSkill \in \Skills$ is the corresponding skill;
%
the \emph{operator parameters} $\DefParametersOf{\operator}{m}$ impose type constraints $\typeOf{\parameterOf{\operator}^i} \subseteq \Types$ on operator arguments;
%
the \emph{preconditions} $\PRE$ are a conjunction of literals over $\Predicates$ defining the conditions necessary to apply the operator;
%
and the \emph{add} and \emph{delete effects}, $\AddEFF$ and $\DeleteEFF$, are the subsets of $\Predicates$ that become true and false, respectively, after the operator is applied.

\paragraph{Grounded Abstractions} To apply an abstract transition model to a real-world setting, the robot must map the low-level state to a high-level abstract state, which requires \emph{grounding} the known predicates using concrete objects so that their truth value may be determined.
%
% To apply the abstract transition model to a real-world setting, an robot needs to appropriately map the state of the real world to an abstract state, which requires determining the truth value of known predicates.
%
A predicate $\predicate \in \Predicates$ may only be grounded using valid arguments, inducing a \emph{grounded predicate} $\DefGroundedPredicate$.
%
Given a low-level state, the classifier \mbox{$\DefGroundedPredicateClassifier$} tests whether the predicate holds for the object arguments.
%
% We can evaluate whether a predicate $\predicate \in \Predicates$ holds for specific objects $\object_{1:n} \in \Objects$ in a state $\state \in \States$ by first \emph{grounding} the predicate by binding the objects comprising that state to the predicate parameters $\ParametersOf{\predicate}$.
%
We define the set of \emph{grounded predicates} for a setting $\DefSetting$ under predicates $\Predicates$ as \mbox{$\DefGroundedPredicates$}, inducing an \emph{abstract state space} $\DefAbstractStates$ where each abstract state corresponds to a specific set of grounded relations.

% The \emph{abstraction function} $\DefAbstractionFunction$ formalizes this relationship by mapping each low-level state $\state \in \States$ to an abstract state $\abstractState \in \AbstractStates$ corresponding to the subset of grounded predicates true in the state.

% \begin{equation}
%     \abstractState = \AbstractionFunction(\state) \triangleq \{ \groundedPredicate \; | \; \groundedPredicate \in \GroundedPredicates \land \GroundedPredicateClassifier(\state) = 1 \}.
% \end{equation}

% David had suggested adding:  where each abstract action corresponds to a black-box skill,

Given a set of operators $\Operators$ in a setting $\DefSetting$, the \emph{abstract action space} $\AbstractActions$ is the set of all valid groundings of the operators using objects from $\Objects$.
%
% The \emph{abstract action space} $\AbstractActions$ is similarly defined by grounding each operator $\operator \in \Operators$ using all valid combinations of objects in the environment.
%
Each \emph{abstract action} (i.e., grounded operator) is defined as $\DefAbstractAction$, where $\operator \in \Operators$, $\NTupleOf{m}{\object} \in \Objects^m$, and for $1 \leq i \leq m$, $\typeOf{\parameterOf{\operator}^i} \subseteq \typeOf{\object_i}$.
%
Grounding an operator induces \emph{ground preconditions} $\GroundPRE$, which are a conjunction of ground literals over $\GroundedPredicates$;
\emph{ground add effects} $\GroundAddEFF \subseteq \GroundedPredicates$;
and \emph{ground delete effects} $\GroundDeleteEFF \subseteq \GroundedPredicates$.

The \emph{grounding function} $\Grounding: \GroundedPredicates \to 2^\States$ maps each grounded predicate to its \emph{grounding set} $\GroundingSetOf{\groundedPredicate} \subseteq \States$, defined as \mbox{$\DefGroundingSet$}.
%
We overload this notation for abstract states $\abstractState \in \AbstractStates$ so that \mbox{$\GroundingSetOf{\abstractState} \Def \bigcap_{\groundedPredicate_i \in \abstractState} \GroundingSetOf{\groundedPredicate_i}$}.
%
Conversely, the \emph{abstraction function} $\Gamma$ maps each low-level state $\state \in \States$ to the abstract state $\abstractState \in \AbstractStates$ defined by \mbox{$\Gamma(\state) \Def \Set{\groundedPredicate \in \GroundedPredicates \SetSuchThat \GroundedPredicateClassifier(\state) = 1}$}.

% An \emph{abstraction function} $\DefAbstractionFunction$ maps each low-level state $\state \in \States$ to an abstract state $\abstractState \in \AbstractStates$ corresponding to the subset of grounded predicates true in the state:

% \begin{equation}
%     \abstractState = \AbstractionFunction(\state) \triangleq \{ \groundedPredicate \; | \; \groundedPredicate \in \GroundedPredicates \land \GroundedPredicateClassifier(\state) = 1 \}.
% \end{equation}

% the \emph{grounding} of an abstract state is the set of low-level states in which all grounded predicates in the abstract state hold.
%
%Finally, the grounding of a set of grounded predicates is the set of low-level states in which all grounded predicates in the set are true.

% $\GroundingSet{\abstractState} = \{ s \in \States \,:\, \forall \groundedPredicate \in \abstractState, \groundedPredicate(s) = 1 \}$

% \textcolor{red}{(Might not be useful anymore since we don't talk about disjunctiveness)In our setting, we assume to have access to a predicate generator $\mathbf{G}$ that proposes predicates $\mathcal{P}$ conditioned on $X \in \mathcal{S}$, such that $\mathcal{G}(\hat{P}) = X$.}

% \subsection{Active Skill Abstraction}
% One aspect that distinguishes our method from Nishanth's papers is the active learning paradigm...

\subsection{Problem Definition}

We now define the task-level model learning problem and a task-level solution as follows: 

\begin{definition}
Given an environment $\DefDomain$ containing settings $\{ \DefSetting \}_{i=1}^N$, we define a \textbf{Task-Level Model Learning} problem as learning an abstract transition model $\DefModel$ for the skills $\Skills$.
\end{definition}

After a period of continual learning in one or more settings, a robot may be evaluated on a \emph{task-level planning problem} $\DefPlanningProblem$, where $\DefGoalStates$ is the set of \emph{goal states} to be reached. 
%
Given a model $\DefModel$, a classical planner can be used to search for an \emph{abstract plan} $\DefAbstractPlan$ that solves the \emph{abstract planning problem} $\DefAbstractPlanningProblem$.
%
\begin{definition}
    An \textbf{abstract plan} $\DefAbstractPlan$ is  a \emph{solution} for skill planning problem \mbox{$\DefPlanningProblem$} iff %, letting $\skillInstance_i$ denote $\skillInstance_{\abstractAction_i}$,
    %
    for $1 \leq i \leq n,\, \state_{i} = \TransitionFunction(\state_{i-1}, \skillInstance_i),
    \state_{i-1} \in \InitiationSetOf{\skillInstance_i},
    \text{ and } \state_n \in \GoalStates,$
    where $\skillInstance_i = \skillInstance_{\abstractAction_i}$.
\end{definition}

% A \emph{solution} to the problem takes the form of a sequence of grounded operators that can map to a \emph{skill plan} (i.e., sequence of skill instances) $\DefPlan$ that reaches a goal state $s_n \in \GoalStates$ from the environment's initial state $\initialState \in \States$.

% \begin{definition}
%     Given an abstract transition model $\mathcal{M}=(\mathcal{P}, \mathcal{A})$ and a skill planning problem $\mathbf{p}$, an \emph{abstract planning problem} requires identifying an abstract plan $[\underline{a}_0, \dots, \underline{a}_{n-1}]$, where $a_i \in \mathcal{A}$, such that the corresponding skill plan $[\skillInstance_0, \dots, \skillInstance_{n-1}]$ is a solution to $\mathbf{p}$.
% \end{definition}

In Sec.~\ref{sec:skillwrapper}, we describe how {\sys} constructs $\gM$ starting with an empty model.


==> sections/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sections/predicate_invention.tex <==
%%% REMEMBER: BENNED WROTE THIS VERSION. PLEASE DO NOT DELETE, BUT WE'RE NOT USING IT FOR CoRL 2026! %%%

% \subsection{Predicate Invention}
% \label{sec:predicate_invention}

% Unlike prior work that requires an initial set of predicates (e.g., goal predicates)~\cite{silver2023predinvent, liang2025visualpredicator, athalye2026pix2pred, liang2025exopredicatorlearningabstractmodels} or partial operators (e.g., with pre-specified effects)~\cite{liang2025visualpredicator, liang2025exopredicatorlearningabstractmodels},
% \sys{} begins without predicates or operators ($\Predicates = \Operators = \emptyset$), instead synthesizing both based on black-box skill executions.

% \paragraph{Conditions for predicate invention.}\,
% \sys{} introduces new predicates only when the current vocabulary is insufficient to distinguish a successful execution
% from a failed execution of the same skill. This provides a \emph{contrastive} signal that a planning-relevant
% condition has gone unexpressed. We identify two such cases: one based on preconditions and the other based on effects.
% % one where the predicates cannot express a skill's preconditions, and one where they cannot express its effects.
% % But they compare different things: the precondition condition compares the pre-states of two transitions, whereas the effect condition compares their effects (i.e., the abstract change from pre- to post-state in each transition).

% \paragraph{Preliminaries}\, %: skill success and the substitution operation.}\,
% Recall that each skill $\skill$ defines a success set $\SuccessSet[\skill] \subseteq \TerminationSet[\skill]$.
% We consider a skill execution \emph{successful} iff it terminates within $\SuccessSet[\skill]$.
% We write $\PreSubgoalSet[\skill]$ to denote the set of states from which $\skill$ succeeds, that is,
% an execution from a state $\state \in \PreSubgoalSet[\skill]$ is exactly one that terminates in
% $\state' \in \SubgoalSet[\skill]$.
% Given a formula $f$ consisting of one or more ground atoms, an object $\object$, and a variable $v$,
% let $f[v/\object]$ denote the result of replacing each occurrence of $\object$ in $f$ with $v$. We can
% extend this to form a \emph{substitution} $\theta = [\bm{v} / \bm{o}]$, where $\bm{v} = \Tuple{v_1, \dots, v_k}$
% and $\bm{o} = \Tuple{o_1, \dots, o_k}$, that replaces each respective object $o_i$ with variable $v_i$.
% We define the \emph{abstract change} between states $\state\in\States$ and $\state'\in\States$ as
% $\Delta(\state, \state') = \Tuple{\AbstractionF(\state') \setminus \AbstractionF(\state), \AbstractionF(\state) \setminus \AbstractionF(\state')}$.
% Finally, let $\abstractState \big|_{\ObjectTuple}$ or $\AbstractionF(\state)\big|_{\ObjectTuple}$ denote the restriction of $\abstractState$ or $\AbstractionF(\state)$, respectively, to include only ground atoms involving at least one object in the tuple $\ObjectTuple$.

% \paragraph{Condition 1 (precondition invention).}\,
% The first condition arises when \sys{} detects that the symbolic vocabulary cannot express a necessary precondition for a skill.
% Concretely, this occurs when two transitions involving instances of the same skill, with one successful and one failed, cannot be distinguished by the current vocabulary.
% We use the substitution operation to account for the fact that the two transitions may involve different skill instances.
% Formally, our condition for precondition invention is:
% \begin{equation}
% \label{eq:precond-invention}
% \begin{aligned}
% &\exists \Tuple{\state_\text{pre}, \skill(\ObjectTuple), \state_\text{post}}, \Tuple{\state_\text{pre}', \skill(\ObjectTuple'), \state_\text{post}'} \in \cD_\skill \text{ s.t. } \state_\text{pre} \in \PreSubgoalSet[\skill(\ObjectTuple)] \text{ and } \state_\text{pre}' \notin \PreSubgoalSet[\skill(\ObjectTuple')], \text{ yet } \\
% &\exists \theta, \theta' \text{ s.t. } [\bm{v} / \ObjectTuple] \subseteq \theta, [\bm{v} / \ObjectTuple'] \subseteq \theta', \text{ and } \theta(\AbstractionF(\state_\text{pre}) \big|_{\ObjectTuple}) = \theta'(\AbstractionF(\state_\text{pre}')\big|_{\ObjectTuple'}),
% \end{aligned}
% \end{equation}
% where % $\ObjectTuple$ denotes the object arguments of $\skill_t(\ObjectTuple)$, $\ObjectTuple'$ denotes the object arguments of $\skill_t(\ObjectTuple')$,
% each of $\theta,\theta'$ is a bijective substitution from objects to variables, $\bm{v}$ is a shared tuple of variables, ensuring that equivalent skill arguments are mapped to the same variables, and $\big|_{\ObjectTuple}$ and $\big|_{\ObjectTuple'}$ restrict the condition to consider only ground atoms involving the object arguments relevant to each transition.

% \paragraph{Condition 2 (effect invention).}\,
% Our second condition detects when the predicate vocabulary cannot express the difference in effects between a successful and a failed execution of a skill:
% %Such cases can be recognized by checking if their effects coincide under the appropriate substitution:
% \begin{equation}
% \label{eq:effect-invention}
% \begin{aligned}
% &\exists \Tuple{\state_\text{pre}, \skill(\ObjectTuple), \state_\text{post}}, \Tuple{\state_\text{pre}', \skill(\ObjectTuple'), \state_\text{post}'} \in \cD_\skill \text{ s.t. } \state_\text{post} \in \SubgoalSet[\skill(\ObjectTuple)] \text{ and } \state_\text{post}' \notin \SubgoalSet[\skill(\ObjectTuple')], \text{ yet } \\
% &\exists \theta, \theta' \text{ s.t. } [\bm{v} / \ObjectTuple] \subseteq \theta, [\bm{v} / \ObjectTuple'] \subseteq \theta', \text{ and } \theta(\Delta(\state_\text{pre}, \state_\text{post}) \big|_{\ObjectTuple}) = \theta'(\Delta(\state_\text{pre}', \state_\text{post}') \big|_{\ObjectTuple'}),
% \end{aligned}
% \end{equation}
% where $\theta $ and $\theta'$ are each a bijective substitution from objects to variables, and $\bm{v}$ is a shared tuple of variables, ensuring that equivalent skill arguments are mapped to the same variables.
% As in Condition 1, we restrict our attention to consider only ground atoms involving skill-relevant objects ($\ObjectTuple$ and $\ObjectTuple'$).


==> sections/problem_setting.tex <==
%
In this section, we briefly discuss our problem setting while defining it formally in Appendix~\ref{app:formal}. 
We consider a robot equipped with a finite set of \emph{object-centric skills} $\Omega$, modeled as black-box options~\citep{sutton1999options}. 
The robot can execute any $\omega \in \Omega$ and determine whether it succeeds, but it does not possess a symbolic transition model of these skills.
Without such a model, the robot cannot plan over a long horizon without reasoning at the low-level state space $\gS$, which is continuous, high-dimensional, and impractical for classical search. 
The goal of \emph{Skill Model Learning} is to acquire a symbolic abstraction of skills that enables efficient composition via classical planning.

\paragraph{Environment} 
An \emph{environment} is a tuple $(\gS, \gT, \Omega, T)$, where $\gS$ is the continuous state space, $\gT$ is a finite set of object types, and $\Omega$ is the skill library. 
Each skill $\omega \in \Omega$ is parameterized by object types drawn from the set $\gT$. 
The environment dynamics are governed by an unknown transition function $T:\gS \times \Omega \to \gS$. 
A \emph{setting} is defined as $(s_0,\gO)$, consisting of an initial state $s_0 \in \gS$ and a set of typed objects $\gO$ with $\tau(o)\subseteq \gT$ for each $o\in\gO$.

\paragraph{Black-box skills} 
A skill $\omega\in\Omega$ is a tuple $(\mathcal{I}_\omega, \pi_\omega, \beta_\omega, \theta_\omega)$, where $\mathcal{I}_\omega \subseteq \gS$ is the \emph{initiation set}, $\pi_\omega$ is the option policy, $\beta_\omega\subseteq\gS$ is the \emph{termination set}, and $\theta_\omega=(\tau^1_\omega,\ldots,\tau^k_\omega)$ are the type constraints on its $k$ parameters. 
A skill instance $\underline{\omega} = \omega(o_1,\ldots,o_k)$ is valid for $o_i \in \gO$ if $\tau^i_\omega \subseteq \tau(o_i)$ for all $i$. 
Executing $\omega$ from $s\in \mathcal{I}_\omega$ terminates in some $s'\in \beta_\omega$, affecting only the state of the bound objects. 

\paragraph{Symbolic predicates and operators} 
To enable abstract reasoning, we introduce a finite set of predicates $\gP$. Each $\sigma \in \gP$ is parameterized by $\gT$ and has a classifier \mbox{$\phi_\sigma: \gO^n \times \gS \rightharpoonup \{0,1\}$} that evaluates its truth value for arguments in a state.
Grounding predicates with valid objects induces a set of grounded predicates $\bar\gP$, and hence an abstract state space $\bar\gS = 2^{\bar\gP}$.
The \emph{abstraction function} $\Gamma:\gS \to \bar\gS$ maps each state to the set of grounded predicates true in that state, while the \emph{grounding function} $\gG:\bar \gS \to \gS$ maps an abstract state to the states in which its grounded predicates hold.

An operator $a \in \gA$ is defined as $(\omega_a, \theta_a, \PRE_a, \EFF_a)$, where $\omega_a \in \Omega$ is the associated skill, $\theta_a$ are typed operator parameters, $\textsc{Pre}_a \subseteq \gP$ is the precondition set, and $\EFF_a = (\AddEFF_a,\DeleteEFF_a)$ are the add and delete effects. 
Grounding all operators $a \in \gA$ with objects $o \in \gO$ yields a set of abstract actions $\bar a\in\bar\gA$, each executable whenever its ground preconditions hold in the current abstract state.

\paragraph{Planning problems} 
Given an environment $(\gS,\gT,\Omega,T)$, the robot’s objective is to learn an abstract transition model 
$\gM = (\gP, \gA)$,
such that $\gM$ is sufficient for planning with $\Omega$. 
Formally, a \emph{skill planning problem} is $(s_0,\gO,\gS_g)$, where $(s_0,\gO)$ is a setting and $\gS_g \subseteq \gS$ are goal states. 
The corresponding \emph{abstract planning problem} is $(\Gamma(s_0),\bar\gA,\bar\gS_g)$, where $\bar\gS_g = \{\bar{s}\in\bar\gS \mid \GroundingSetOf{\bar{s}}\cap \gS_g \neq\emptyset\}$.
An abstract plan $\bar \pi = \langle \bar{a}_1,\ldots,\bar{a}_n\rangle$ is \emph{valid} if its execution under $\gM$ yields an abstract trajectory consistent with some feasible low-level trajectory under $T$, ending in a goal state.

\paragraph{Problem statement} 
The \emph{Skill Model Learning} problem is: given experience in the form of \textit{state}–\textit{skill-instance}–\textit{next-state} tuples $\langle s,\underline{\omega},s'\rangle$, learn a model $\gM=(\gP,\gA)$ such that every plan found by a complete symbolic planner over $\gM$ corresponds to a feasible low-level skill plan.

